How Do Fair Decisions Fare in Long-term Qualification?

Although many fairness criteria have been proposed for decision making, their long-term impact on the well-being of a population remains unclear. In this work, we study the dynamics of population qualification and algorithmic decisions under a partially observed Markov decision problem setting. By characterizing the equilibrium of such dynamics, we analyze the long-term impact of static fairness constraints on the equality and improvement of group well-being. Our results show that static fairness constraints can either promote equality or exacerbate disparity depending on the driving factor of qualification transitions and the effect of sensitive attributes on feature distributions. We also consider possible interventions that can effectively improve group qualification or promote equality of group qualification. Our theoretical results and experiments on static real-world datasets with simulated dynamics show that our framework can be used to facilitate social science studies.

==> app_generation.tex <==
\section{Impact of decisions on generation process}\label{sec:generation}
\subsection{Results}
In this section we consider
the scenario where institute's decision not only affects the transition of the qualification state but also affects the generation process of individual feature $X_t$. We will only focus on analyzing its impact on equilibrium under unconstrained policy, the analysis only involves one group. Therefore, we remove the subscript $s\in\{a,b\}$ in this section. Let the generation probability distribution be  $G_{yd}(x) \coloneqq \mathbb{P}(X_t = x \mid Y_t= y, D_{t-1}=d)$ and corresponding CDF be $\mathbb{G}_{yd}(x)$. 

Denote $\zeta^{yd}_t \coloneqq \mathbb{P}(D_{t-1}=d,Y_t = y)$, then qualification profile $\gamma_t(x) =  \frac{1}{1 + 
\frac
{G_{00}(x) \zeta^{00}_t+G_{01}(x) \zeta^{01}_t}
{G_{10}(x) \zeta^{10}_t+G_{11}(x) \zeta^{11}_t}
}$ and qualification rate $\alpha_t = \zeta_t^{11}+\zeta_t^{10}$. See Appendix \ref{app:generation} for derivations and dynamics of $\alpha_t$. 

\begin{assumption}\label{ass:3}
$\frac{G_{00}(x)}{G_{10}(x)}$, $\frac{G_{00}(x)}{G_{11}(x)}$, $\frac{G_{01}(x)}{G_{10}(x)}$,
$\frac{G_{01}(x)}{G_{11}(x)}$ are continuous and strictly decreasing in $x$.
\end{assumption}

Under Assumption \ref{ass:3}, given $\{\zeta^{yd}_{t}\}_{y,d}$, $\gamma_t(x)$ is strictly increasing in $x$ and unconstrained optimal policy is threshold policy. In the following we focus on a special case where decision only affect feature of (un)qualified people, i.e., $G_{01}(x) \neq G_{00}(x), G_{11}(x) = G_{10}(x) = G_1(x)$ or $G_{11}(x) \neq G_{10}(x), G_{01}(x) = G_{00}(x) = G_0(x)$. We wonder as compared to the case when $G_{y1}(x) = G_{y0}(x), \forall y=0,1$ (main body of the paper), how is the equilibrium under unconstrained optimal policies affected in these cases.

\begin{assumption}\label{ass:generation_1}
$\mathbb{G}_{01}(x) \leq \mathbb{G}_{00}(x),\forall x$ and $\exists$ a unique $\widehat{x}$ such that ${G}_{01}(\widehat{x}) = {G}_{00}(\widehat{x})$, ${G}_{01}(x) < {G}_{00}(x), \forall x < \widehat{x}$, ${G}_{01}(x) > {G}_{00}(x), \forall x > \widehat{x}$. 
\end{assumption}
\begin{assumption}\label{ass:generation_2}
$\mathbb{G}_{01}(x) \geq \mathbb{G}_{00}(x), \forall x$ and $\exists$ a unique $\widehat{x}$ such that ${G}_{01}(\widehat{x}) = {G}_{00}(\widehat{x})$, ${G}_{01}(x) > {G}_{00}(x), \forall x < \widehat{x}$, ${G}_{01}(x) < {G}_{00}(x), \forall x > \widehat{x}$.
\end{assumption}
\begin{theorem}\label{thm:generation}
Consider two scenarios with the same set of transitions $\{T_{yd}\}_{y,d}$ and the same $G_{11}(x) = G_{10}(x)$: scenario $A$ has distributions $G^A_{00}(x) \neq G^A_{01}(x)$ and scenario $B$ has $G^B_{00}(x) = G^B_{01}(x) = G^A_{01}(x)$. Let $\widehat{\alpha}_B$ be the unique equilibrium of scenario $B$. Then under Assumption \ref{ass:3}, scenario $A$ has at least one equilibrium $\widehat{\alpha}_A$. Moreover, if $\frac{u_+}{u_-}>\frac{G_{01}^A(\widehat{x})}{G_{11}(\widehat{x})}\max\{\frac{1-T_{10}}{T_{00}},\frac{1-T_{11}}{T_{01}}\}$, we have:
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item Under Assumption \ref{ass:generation_1}, we have $\widehat{\alpha}_A > \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_I};  $\widehat{\alpha}_A < \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_II}. 
    \item Under Assumption \ref{ass:generation_2}, we have $\widehat{\alpha}_A < \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_I};  $\widehat{\alpha}_A > \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_II}. 
\end{itemize}
\end{theorem}
\begin{figure}[H]
\centering
\includegraphics[trim=0cm 0cm 0cm 1.4cm,clip=true,width=0.37\textwidth]{plots/comDiff.pdf}
\includegraphics[trim=0cm 0cm 0cm 1.4cm,clip=true,width=0.37\textwidth]{plots/comDiff1.pdf}
\caption{Illustration of feature distributions in two scenarios:
the left plot shows the case when $\mathbb{G}_{01}^A(\theta)\leq \mathbb{G}_{00}^A(\theta), \forall \theta$, with $G_{00}^A(X)\sim \mathcal{N}(-8,9)$, $G_{01}^A(X)\sim \mathcal{N}(-1,9)$; the right plot shows the case when $\mathbb{G}_{01}^A(\theta)\geq \mathbb{G}_{00}^A(\theta), \forall \theta$, with $G_{00}^A(X)\sim \mathcal{N}(-1,9)$, $G_{01}^A(X)\sim \mathcal{N}(-8,9)$.
Moreover, $G_{1}(X)\sim \mathcal{N}(5,9)$, 
$\zeta^{00} = 0.2$, $\alpha = 0.4$ in both cases. Within each plot, the upper and lower subplots show distributions in scenario $B$ and $A$ respectively.}
\label{fig:diff_ill}
\end{figure}
Similar results can be concluded for case when $G_{11}(x) \neq G_{10}(x), G_{01}(x) = G_{00}(x) = G_0(x)$.


\begin{assumption}\label{ass:generation1}
$\mathbb{G}_{11}(x) \leq \mathbb{G}_{10}(x),\forall x$ and $\exists$ a unique $\widehat{x}$ such that ${G}_{11}(\widehat{x}) = {G}_{10}(\widehat{x})$, ${G}_{11}(x) < {G}_{10}(x), \forall x < \widehat{x}$, ${G}_{11}(x) > {G}_{10}(x), \forall x > \widehat{x}$. 
\end{assumption}
\begin{assumption}\label{ass:generation2}
$\mathbb{G}_{11}(x) \geq \mathbb{G}_{10}(x), \forall x$ and $\exists$ a unique $\widehat{x}$ such that ${G}_{11}(\widehat{x}) = {G}_{10}(\widehat{x})$, ${G}_{11}(x) > {G}_{10}(x), \forall x < \widehat{x}$, ${G}_{11}(x) < {G}_{10}(x), \forall x > \widehat{x}$.
\end{assumption}
\begin{theorem}\label{thm:generation1}
Consider two scenarios with the same set of transitions $\{T_{yd}\}_{y,d}$ and the same $G_{01}(x) = G_{00}(x)$: scenario $A$ has distributions $G^A_{10}(x) \neq G^A_{11}(x)$ and scenario $B$ has $G^B_{10}(x) = G^B_{11}(x) = G^A_{10}(x)$. Let $\widehat{\alpha}_B$ be the unique equilibrium of scenario $B$. Then under Assumption \ref{ass:3}, scenario $A$ has at least one equilibrium $\widehat{\alpha}_A$. Moreover, if $\frac{u_+}{u_-}<\frac{G_{00}(\widehat{x})}{G^A_{10}(\widehat{x})}\min\{\frac{1-T_{10}}{T_{00}},\frac{1-T_{11}}{T_{01}}\}$, we have
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
\item Under Assumption \ref{ass:generation1}, we have $\widehat{\alpha}_A < \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_I}; $\widehat{\alpha}_A > \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_II}.
\item Under Assumption \ref{ass:generation2}, we have $\widehat{\alpha}_A > \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_I}; $\widehat{\alpha}_A < \widehat{\alpha}_B$ under Condition \ref{con:transition}\ref{con:transition_II}.
\end{itemize}
\end{theorem}

\subsection{Derivations}\label{app:generation}
\paragraph{Qualification profile.}
\begin{eqnarray} \label{eq:qlfn_profile_gen}
\gamma_t(x) &=& \mathbb{P}(Y_t = 1|X_t = x) %= \frac{\mathbb{P}(Y_t = 1, X_t = x)}{\mathbb{P}(Y_t = 1, X_t = x) + \mathbb{P}(Y_t = 0, X_t = x)} 
=  \frac{1}{1 + \frac{\mathbb{P}(Y_t = 0, X_t = x)}{\mathbb{P}(Y_t = 1, X_t = x)}} \nonumber \\
&=&  \frac{1}{1 + \frac{
\sum_{d}\mathbb{P}(X_t = x\mid D_{t-1}=d, Y_t = 0 )\mathbb{P}(D_{t-1}=d,Y_t = 0)}{
\sum_{d}\mathbb{P}(X_t = x \mid D_{t-1}=d,Y_t = 1 )\mathbb{P}(D_{t-1}=d,Y_t = 1)}} \nonumber 
\\&=&  \frac{1}{1 + 
\frac
{G_{00}(x) \zeta^{00}_t+G_{01}(x) \zeta^{01}_t}
{G_{10}(x) \zeta^{10}_t+G_{11}(x) \zeta^{11}_t}
}.\nonumber
\end{eqnarray}

\paragraph{Dynamics of qualification rate}

\begin{eqnarray*} \label{eq:dynamics_gen}
\zeta^{yd}_t &=& \mathbb{P}(D_{t-1}=d,Y_t = y) \\&=& \sum_{d',y'} 
\mathbb{P}(Y_t = y, D_{t-1}=d \mid Y_{t-1}=y, D_{t-2}=d') 
\mathbb{P}(Y_{t-1}=y', D_{t-2}=d')\nonumber \\
& = & \sum_{d',y'} 
\mathbb{P}(Y _{t-1}=y', D_{t-2}=d')
\mathbb{P}(Y_t = y \mid  D_{t-1}=d , Y_{t-1}=y')\\&&
\mathbb{P}( D_{t-1}=d \mid Y_{t-1} = y', D_{t-2} = d' )
\nonumber \\
&=& \sum_{d',y'} 
\mathbb{P}(Y _{t-1}=y', D_{t-2}=d')
\mathbb{P}(Y_t = y \mid  D_{t-1}=d , Y_{t-1}=y') \nonumber \\
&& \int \mathbb{P}( D_{t-1}=d \mid X_{t-1} = x')\mathbb{P}( X_{t-1}=x \mid Y_{t-1} = y', D_{t-2} = d' ) dx'. 
\end{eqnarray*}
Simplify notation $\mathbb{E}_{X_{t-1} \mid Y_{t-1}=y',D_{t-2}=d'}[\cdot]$ as $\mathbb{E}^{y'd'}[\cdot]$,
and $\pi_{t-1}(X_{t-1})$ as $\pi$. Evolution equation is given as:
\begin{eqnarray*}
\zeta_t = \Gamma_{t-1}\zeta_{t-1}.
\end{eqnarray*}
where $\zeta_t = \begin{bmatrix}
\zeta^{11}_{t}&
\zeta^{10}_{t}&
\zeta^{01}_{t}&
\zeta^{00}_{t}
\end{bmatrix}^T$ and
\begin{eqnarray*} 
\Gamma_{t-1} = 
\begin{bmatrix}
T_{11}\mathbb{E}^{11}[\pi] & T_{11}\mathbb{E}^{10}[\pi] &
T_{01}\mathbb{E}^{01}[\pi] & T_{01}\mathbb{E}^{00}[\pi]\\
T_{10}\mathbb{E}^{11}[1-\pi] & T_{10}\mathbb{E}^{10}[1-\pi] &
T_{00}\mathbb{E}^{01}[1-\pi] & T_{00}\mathbb{E}^{00}[1-\pi]\\
(1-T_{11})\mathbb{E}^{11}[\pi] & (1-T_{11})\mathbb{E}^{10}[\pi] &
(1-T_{01})\mathbb{E}^{01}[\pi] & (1-T_{01})\mathbb{E}^{00}[\pi]\\
(1-T_{10})\mathbb{E}^{11}[1-\pi] &(1-T_{10})\mathbb{E}^{10}[1-\pi] &
(1-T_{00})\mathbb{E}^{01}[1-\pi] &(1-T_{00})\mathbb{E}^{00}[1-\pi]\\
\end{bmatrix}
\end{eqnarray*}
Qualification rate satisfies $\alpha_t = \zeta_t^{11}+\zeta_t^{10}$.

\subsection{Proof}
\input{proofs/prf_thm5}

==> plots/fico.tex <==
\begin{tikzpicture}
\begin{axis}[
xmin = -4, xmax = 4,
ymin = -4, ymax = 4,
zmin = 0, zmax = 1,
axis equal image,
view = {0}{90},
]
\addplot3[
quiver = {
u = {-y},
v = {x},
},
-stealth,
domain = -4:4,
domain y = -4:4,
] {0};
\end{axis}
\end{tikzpicture}

==> plots/fico_ne.tex <==
\usepgflibrary{arrows} % LATEX and plain TEX and pure pgf 
\usepgflibrary[arrows] % ConTEXt and pure pgf 
\usetikzlibrary{arrows} % LATEX and plain TEX when using TikZ 
\usetikzlibrary{arrows.meta}

\usetikzlibrary[arrows] % ConTEXt when using TikZ
\begin{tikzpicture}
\begin{axis}[
axis equal,
xmin=0, xmax=1,
ymin=0,ymax=1,
scatter/classes={a={mark=o,draw=black}},
xlabel={$x$},
ylabel={$y$},
scale=1
]
\addplot[
scatter,
only marks,
mark size = 2pt,
fill = red,
scatter src=explicit symbolic]
coordinates { 
(0.1693273561013531,0.21833386435466112)
(0.17979083705314974,0.2600148969927734)
(0.1927457873239222,0.32584071171473683)
(0.20948176708271016,0.425854010310586)

(0.21562261719856365,0.28647531105490176)
(0.2346289171072899,0.34608412690694323)
(0.25954218448981936,0.43047964505523495)
(0.2935659294034017,0.5411437437641949)

(0.2836558725151473,0.36673019992347655)
(0.3171782468301674,0.43925016808385015)
(0.36211954695762777,0.5311515138382906)
(0.4240011055965353,0.6363309595643126)

(0.3757846811772098,0.4500435480098369)
(0.42796064621191854,0.5275572852552228)
(0.4963549114224435,0.6161704486021093)
(0.5859167114822401,0.7065596440462895)
};
\addplot [->, thick,  black]
coordinates { (0.1,0.2) (0.3,0.4)};
\draw[->](0,0) -- (1,1);

\end{axis}
\end{tikzpicture}

==> proofs/prf_prop4.tex <==
% \section{An example of the generalization to high-dimensional feature space}
% The results above can be generalized to high-dimensional feature space where $X\in \mathbb{R}^d$. We consider a comprehensive class of feature generation distributions and suppose $\forall s\in \{a,b\}, \forall y\in \{0,1\}$, distribution of $X|Y=y,S=s$ belongs to exponential family and can be written as $G_y^s(x) \coloneqq B(x)\exp\big(\langle\eta(\omega_y^s),\xi(x)\rangle-A(\omega_y^s)\big)$ where $\langle x,y \rangle$ represents inner product of two vectors $x,y$. Then $\frac{G_0^s(x)}{G_1^s(x)} = \exp\big( -\langle \eta^s,\xi(x)\rangle + A^s\big)$ where $\eta^s \coloneqq \eta(\omega_1^s)-\eta(\omega_0^s)$ and $A^s \coloneqq A(\omega_1^s)-A(\omega_0^s)$.

% Let threshold function policy parameterized by $\theta^s\in \mathbb{R}$ be defined as $\pi^s(x) = \textbf{1}(\langle \eta^s,\xi(x)\rangle \geq \theta^s)$.
% \begin{proposition}[Threshold function policies are optimal]\label{prop:highDim}
% Unconstrained, \texttt{DP} and \texttt{EqOpt} fair optimal myopic policies are all threshold function policies, i.e., $\forall x,t$ and $s\in \{a,b\}$, $\pi^s_t(x) = \textbf{1}(\langle \eta^s,\xi(x)\rangle \geq \theta^s_t)$ for some $\theta^s_t \in \mathbb{R}$.
% \end{proposition}
% In high-dimensional settings, under the policy $\pi^s(x) = \textbf{1}(\langle \eta^s,\xi(x)\rangle \geq \theta^s)$, define a set $\mathcal{S}(\theta^s) \coloneqq \{x: \langle \eta^s,\xi(x)\rangle \geq \theta^s, x\in \mathbb{R}^d\}$, then $\mathbb{E}_{X_t\mid Y_t=y,S=s}\Big[\pi_t^s(X_t)\Big] = \int_{x\in\mathcal{S}(\theta^s)}G_y^s(x)dx$ is non-increasing in $\theta^s$. In dynamics \eqref{eq:dynamics}, $g_t^{ys} = T^s_{y0}\int_{x\in\mathcal{S}(\theta^s_t)}G_y^s(x)dx + T^s_{y1}(1-\int_{x\in\mathcal{S}(\theta^s_t)}G_y^s(x)dx)$. All analysis for one-dimensional setting are still valid by replacing notation $\mathbb{G}^y_s(\theta^s)$ as $\int_{x\in\mathcal{S}(\theta^s)}G_y^s(x)dx$. 

% \begin{example}
%  Let $X\mid Y=y,S=s$ follows $d$-dimensional normal distribution $\mathcal{N}(\mu^s_y,\Sigma^s_y)$, $\forall s\in \{a,b\}, \forall y\in\{0,1\}$, then it belongs to exponential family with $B(x) = (2\pi)^{-d/2}|(\Sigma^s_y)^{-1}|^{1/2}$ and
% \begin{eqnarray*}
% \xi(x) = \begin{bmatrix}
% x\\
% xx^T
% \end{bmatrix};& \eta(\mu^s_y,\Sigma^s_y) = \begin{bmatrix}
% (\Sigma^s_y)^{-1}\mu^s_y\\
% -\frac{1}{2}(\Sigma^s_y)^{-1}
% \end{bmatrix}; & A( \mu^s_y,\Sigma^s_y) = \frac{1}{2}(\mu^s_y)^T(\Sigma^s_y)^{-1}\mu^s_y.
% \end{eqnarray*}
% Therefore, $\frac{G^s_0(x)}{G^s_1(x)} = \exp\big( -\langle \eta^s,\xi(x)\rangle + A^s\big)$ with
% \begin{eqnarray}
% \eta^s = \begin{bmatrix}
% (\Sigma^s_1)^{-1}\mu^s_1-(\Sigma^s_0)^{-1}\mu^s_0\\
% -\frac{1}{2}(\Sigma^s_1)^{-1}+\frac{1}{2}(\Sigma^s_0)^{-1}
% \end{bmatrix}; & A^s = \frac{1}{2}\Big((\mu^s_1)^T(\Sigma^s_1)^{-1}\mu^s_1-(\mu^s_0)^T(\Sigma^s_0)^{-1}\mu^s_0\Big).
% \end{eqnarray}
% \end{example}
\paragraph{The proof of Proposition \ref{prop:highDim}}
\begin{proof}
The proof follows the same idea as Lemma \ref{lemma:optimal_threshold_form}. We omit the subscript $t$. 

The unconstrained optimal policy satisfies $\pi^s_{\texttt{UN}}(x) = \textbf{1}(\gamma^s(x)\geq \frac{c}{b+c}) = \textbf{1}\Big(\frac{G^s_0(x)}{G^s_1(x)}\leq \frac{b}{c}\frac{\alpha}{1-\alpha}\Big)$. Plug in $\frac{G_0^s(x)}{G_1^s(x)} = \exp\big( -\langle \eta^s,\xi(x)\rangle + A^s\big)$, we have $\pi^s_{\texttt{UN}}(x) = \textbf{1}\Big( \langle \eta^s,\xi(x)\rangle \geq A^s - \log\big( \frac{b}{c}\frac{\alpha}{1-\alpha}\big) \Big) $, which is threshold function policy with threshold $\theta^s_{\texttt{UN}} = A^s - \log\big( \frac{b}{c}\frac{\alpha}{1-\alpha}\big)$.

For the optimal fair policy, similar to proof of Lemma \ref{lemma:optimal_threshold_form}, we consider any pair of policies $(\pi^a,\pi^b)$ that satisfies fairness constraint $\mathcal{C}$, and show that there always exists a pair of threshold function policies $(\pi^a_d,\pi^b_d)$ such that $\mathbb{E}_{X\sim \mathcal{P}_{\mathcal{C}}^s}[\pi^s(X)] = \mathbb{E}_{X\sim \mathcal{P}_{\mathcal{C}}^s}[\pi^s_d(X)] $ and the utility of $\pi^s_d$ is no less than the utility attained under $\pi^s$.

$\forall s\in \{a,b\}$, let threshold function policy be defined such that $\pi^s_d(x) = \textbf{1}(\langle \eta^s,\xi(x)\rangle \geq \theta_d^s)$ and $\mathbb{E}_{X\sim \mathcal{P}_{\mathcal{C}}^s}[\pi^s(X)] = \mathbb{E}_{X\sim \mathcal{P}_{\mathcal{C}}^s}[\pi^s_d(X)] = c$. If CDF of $\mathcal{P}_{\mathcal{C}}^s$ is continuous, then such threshold function policy must exist. Next we show that $\forall s \in \{a,b\}$, $\mathbb{E}_{X|S=s}[\pi^{s}_d(X)(\gamma^s(X)(b+c) -c) ]\geq  \mathbb{E}_{X|S=s}[\pi^{s}(X)(\gamma^s(X)(b+c) -c) ]$ holds. 

Define two sets $\mathcal{S}^{+} \coloneqq \{x: \langle \eta^s,\xi(x)\rangle \geq \theta_d^s, x\in \mathbb{R}^d\}$ and $\mathcal{S}^{-} \coloneqq \{x: \langle \eta^s,\xi(x)\rangle < \theta_d^s, x\in \mathbb{R}^d\}$, then
\begin{eqnarray*}
\mathbb{E}_{X|S=s}[\pi^{s}_d(X)(\gamma^s(X)(b+c) -c) ] &=& \int_{x\in \mathcal{S}^{+}}(\gamma^s(x)(b+c) -c)\mathbb{P}(X=x\mid S=s) dx\\
\mathbb{E}_{X|S=s}[\pi^{s}(X)(\gamma^s(X)(b+c) -c) ]&=& \int_{x\in \mathcal{S}^{+}}(\gamma^s(x)(b+c) -c)\mathbb{P}(X=x\mid S=s) dx\\
&&+\int_{x\in \mathcal{S}^{-}}\pi^s(x)(\gamma^s(x)(b+c) -c)\mathbb{P}(X=x\mid S=s) dx\\
&&-\int_{x\in \mathcal{S}^{+}}(1-\pi^s(x))(\gamma^s(x)(b+c) -c)\mathbb{P}(X=x\mid S=s) dx
\end{eqnarray*}
Because 
\begin{eqnarray*}
(\gamma^s(x)(b+c) -c)\frac{\mathbb{P}(X=x\mid S=s)}{\mathcal{P}^s_{\mathcal{C}}(x)}
 &= &
\alpha^s \frac{G^s_1(x)}{\mathcal{P}^s_{\mathcal{C}}(x)} b -
(1-\alpha^s)\frac{G^s_0(x)}{\mathcal{P}^s_{\mathcal{C}}(x)}c \\
&=&\begin{cases}
\alpha^s b -
(1-\alpha^s)\frac{G^s_0(x)}{G^s_1(x)}c, \text{   if }\mathcal{C} =  \texttt{EqOpt}\\
 \frac{1}{1+\frac{1-\alpha^s}{\alpha^s}\frac{G^s_0(x)}{G^s_1(x)}} b -
\frac{1}{\frac{\alpha^s}{1-\alpha^s}\frac{G^s_1(x)}{G^s_0(x)}+1}c, \text{   if } \mathcal{C} =  \texttt{DP}
\end{cases}
\end{eqnarray*}
is decreasing in $\frac{G_0^s(x)}{G_1^s(x)}$ and  $\frac{G_0^s(x)}{G_1^s(x)} = \exp\big( -\langle \eta^s,\xi(x)\rangle + A^s\big)$ is strictly decreasing in $\langle \eta^s,\xi(x)\rangle$, it implies that $(\gamma^s(x)(b+c) -c)\frac{\mathbb{P}(X=x\mid S=s)}{\mathcal{P}^s_{\mathcal{C}}(x)}$ is strictly increasing in $\langle \eta^s,\xi(x)\rangle$. 

Because of fairness constraint, we have
\begin{eqnarray*}
\int_{x\in \mathcal{S}^{+}}(1-\pi^{s}(x))\mathcal{P}^s_{\mathcal{C}}(x)dx = \int_{x\in \mathcal{S}^{-}}\pi^{s}(x)\mathcal{P}^s_{\mathcal{C}}(x)dx
\end{eqnarray*}
Therefore, the followings hold under $\mathcal{C} = \texttt{EqOpt}$ or \texttt{DP},
\begin{eqnarray*}
&&\int_{x\in \mathcal{S}^{-}}\pi^{s}(x)(\gamma^s(x)(b+c) -c)\mathbb{P}(X=x\mid S=s) dx \\ &=& \int_{x\in \mathcal{S}^{-}}\pi^{s}(x)(\gamma^s(x)(b+c) -c)\frac{\mathbb{P}(X=x\mid S=s)}{\mathcal{P}^s_{\mathcal{C}}(x)}\mathcal{P}^s_{\mathcal{C}}(x) dx \\
&\leq&
\int_{x\in \mathcal{S}^{-}}\pi^{s}(x)
(\gamma^s(x^*)(b+c) -c)\frac{\mathbb{P}(X=x^*\mid S=s)}{\mathcal{P}^s_{\mathcal{C}}(x^*)}
\mathcal{P}^s_{\mathcal{C}}(x) dx \\
&=&
\int_{x\in \mathcal{S}^{+}}(1-\pi^{s}(x))
(\gamma^s(x^*)(b+c) -c)\frac{\mathbb{P}(X=x^*\mid S=s)}{\mathcal{P}^s_{\mathcal{C}}(x^*)}
\mathcal{P}^s_{\mathcal{C}}(x) dx\\
&\leq&\int_{x\in \mathcal{S}^{+}}(1-\pi^{s}(x))(\gamma^s(x)(b+c) -c)\frac{\mathbb{P}(X=x\mid S=s)}{\mathcal{P}^s_{\mathcal{C}}(x)}\mathcal{P}^s_{\mathcal{C}}(x) dx\\
&=&\int_{x\in \mathcal{S}^{+}}(1-\pi^{s}(x))(\gamma^s(x)(b+c) -c)\mathbb{P}(X=x\mid S=s) dx.
\end{eqnarray*}
where $x^*$ is defined such that $ \langle \eta^s,\xi(x^*)\rangle = \theta^s_d$. Therefore, $\forall s\in \{a,b\}$, $\mathbb{E}_{X|S=s}[\pi^{s}_d(X)(\gamma^s(X)(b+c) -c) ]\geq  \mathbb{E}_{X|S=s}[\pi^{s}(X)(\gamma^s(X)(b+c) -c) ]$, i.e., the utility attained under threshold function policy $(\pi^a_d,\pi^b_d)$ is no less than the utility of $(\pi^a,\pi^b)$, which concludes that the optimal fair policy $(\pi^a_{\mathcal{C}},\pi^b_{\mathcal{C}})$ must be threshold function policies.
\end{proof}

==> proofs/prf_thm5.tex <==

\paragraph{The Proof of Theorem \ref{thm:generation}.}
\begin{proof}
In the proof, let $G_{11}(x) = G_{10}(x) = G_1(x)$ and remove subscript $A$ to simplify the notation, i.e., ${G}_{0d}^A(\theta)\coloneqq {G}_{0d}(\theta)$, $\forall d\in\{0,1\}$. 

Under Assumption \ref{ass:3} and the case when $G_{11}(x) = G_{10}(x) = G_{1}(x)$, $G_{01}(x) \neq G_{00}(x)$, use the fact that $\zeta^{11}_t + \zeta^{10}_t = \alpha_t$, $\zeta^{11}_t + \zeta^{10}_t +\zeta^{01}_t + \zeta^{00}_t = 1$, dynamics of qualification rate can be simplified as follows, where $\theta_t$ is the threshold of the policy at $t$. 
\begin{eqnarray*}
\alpha_{t+1} &=& [T_{11}(1-\mathbb{G}_{1}(\theta_t))+T_{10}\mathbb{G}_{1}(\theta_t) - T_{01}(1-\mathbb{G}_{01}(\theta_t))-T_{00}\mathbb{G}_{01}(\theta_t)]\alpha_{t} \\
&&+ T_{01} (1-\mathbb{G}_{01}(\theta_t)) + T_{00}\mathbb{G}_{01}(\theta_t)+(\mathbb{G}_{01}(\theta_t)-\mathbb{G}_{00}(\theta_t))(T_{01}-T_{00})\zeta^{00}_t\\
\zeta^{00}_{t+1} &=& [(1-T_{10})\mathbb{G}_{1}(\theta_t) - (1-T_{00})\mathbb{G}_{01}(\theta_t)]\alpha_t + (1-T_{00})[\mathbb{G}_{01}(\theta_t)(1-\zeta^{00}_{t})+\mathbb{G}_{00}(\theta_t)\zeta^{00}_{t} ]
\end{eqnarray*}
and qualification profile is reduced to $\gamma_t(x) =  \frac{1}{1 + 
\frac
{G_{00}(x) \zeta^{00}_t+G_{01}(x) \zeta^{01}_t}
{G_{1}(x) \alpha_t}
}$.

The scenario $A$ has the equilibrium if there exists $\alpha$, $\zeta^{00}$ such that the following holds:
\begin{eqnarray*}
\alpha &=& [T_{11}(1-\mathbb{G}_{1}(\theta))+T_{10}\mathbb{G}_{1}(\theta) - T_{01}(1-\mathbb{G}_{01}(\theta))-T_{00}\mathbb{G}_{01}(\theta)]\alpha \nonumber \\
&&+ T_{01} (1-\mathbb{G}_{01}(\theta)) + T_{00}\mathbb{G}_{01}(\theta)+(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{01}-T_{00})\zeta^{00}\label{eq:alpha}\\
\zeta^{00} &=& [(1-T_{10})\mathbb{G}_{1}(\theta) - (1-T_{00})\mathbb{G}_{01}(\theta)]\alpha + (1-T_{00})[\mathbb{G}_{01}(\theta)(1-\zeta^{00})+\mathbb{G}_{00}(\theta)\zeta^{00} ]\nonumber\label{eq:zeta}
\end{eqnarray*}
Re-organize above equations,
\begin{eqnarray*}
\frac{1}{\alpha}- 1 &=& \resizebox{0.8\hsize}{!}{$\frac{1-T_{11}(1-\mathbb{G}_{1}(\theta))-T_{10}\mathbb{G}_{1}(\theta)-(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{01}-T_{00})\zeta^{00}}{T_{01}(1-\mathbb{G}_{01}(\theta))+T_{00}\mathbb{G}_{01}(\theta)+(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{01}-T_{00})\zeta^{00}}= h_A(\theta_A(\zeta^{00},\alpha))\label{eq:alpha1}$}\\
\zeta^{00} &=& \frac{[(1-T_{10})\mathbb{G}_1(\theta)-(1-T_{00})\mathbb{G}_{01}(\theta)]\alpha+(1-T_{00})\mathbb{G}_{01}(\theta) }{1+(1-T_{00})(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))} = g_A(\theta_A(\zeta^{00},\alpha))
\end{eqnarray*}
%Take derivative of the $h(\theta)$ w.r.t. $\theta$ gives $\frac{d h(\theta)}{d \theta} =$
%\begin{eqnarray*}
% \frac{1}{g(\theta)^2}\Big[(T_{11}-T_{01})G_1(\theta)\underbrace{\Big(T_{10}(1-\mathbb{G}_{01}(\theta)) + T_{00}\mathbb{G}_{01}(\theta)+(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{10}-T_{00})\zeta^{00}\Big)}_{\textbf{term 1}} \\
%+(T_{10}-T_{00})\underbrace{G_{01}(\theta)\Big((1-\zeta^{00})(1-T_{11}(1-\mathbb{G}_{1}(\theta)) - T_{01}\mathbb{G}_{1}(\theta))+\mathbb{G}_{00}(\theta)(T_{10}-T_{00})\zeta^{00}-\zeta^{00}T_{10} \Big)}_{\textbf{term 2}}\\
%+ (T_{10}-T_{00})\underbrace{G_{00}(\theta)\zeta^{00}\Big(T_{10}(1-\mathbb{G}_{01}(\theta))+T_{00}\mathbb{G}_{01}(\theta)+1-T_{11}(1-\mathbb{G}_1(\theta))-T_{01}\mathbb{G}_1(\theta) \Big)}_{\textbf{term 3}}\Big]
%\end{eqnarray*}
%where $g(\theta) = T_{10}(1-\mathbb{G}_{01}(\theta))+T_{00}\mathbb{G}_{01}(\theta)+(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{10}-T_{00})\zeta^{00}$.
%\begin{eqnarray*}
%\textbf{term 1} &=& %\mathbb{G}_{01}(\theta)(T_{10}-T_{00})(\zeta^{00}-1) + T_{10} - %\mathbb{G}_{00}(\theta)\zeta^{00}(T_{10}-T_{00%})\\
%&\geq& -(1-\zeta^{00})(T_{10}-T_{00}) + T_{10} %- \zeta^{00}(T_{10}-T_{00})= T_{00} > 0\\
%\textbf{term 2} %&>&-G^{01}(\theta)\zeta^{00}T_{10}\\
%\textbf{term 3} %&>&G^{00}(\theta)\zeta^{00}(1-T_{11}+T_{00}) 
%\end{eqnarray*}
where $\theta \coloneqq \theta_A(\zeta^{00},\alpha)$ in equations for simplification. Given any $\zeta^{00}$, $h_A(\theta_A(\zeta^{00},\alpha))$ is continuous in $\alpha$, there exists at least one $\overline{\alpha} \coloneqq \psi(\zeta^{00})$ such that $\frac{1}{\overline{\alpha}}-1 = h_A(\theta_A(\zeta^{00},\overline{\alpha}))$ holds. 


Given any $\alpha\in [0,1]$, $g_A(\theta_A(\zeta^{00},\alpha))\in (0,1)$ is continuous in $\zeta^{00}$, while $\zeta^{00}$ is strictly increasing from 0 to 1. Therefore, there exists at least one $\overline{\zeta}^{00}\coloneqq \eta(\alpha)$ such that $\overline{\zeta}^{00} =  g_A(\theta_A(\overline{\zeta}^{00},\alpha))$. 

Consider a 2D plane $\{(\alpha,\zeta^{00}):\zeta^{00}\in [0,1],\alpha\in[0,1]\}$, two sets of curves $\mathcal{C}_1 = \{(\alpha,\zeta^{00}):\alpha = \psi(\zeta^{00}),\zeta^{00}\in (0,1)\}$ and $\mathcal{C}_2 = \{(\alpha,\zeta^{00}):\zeta^{00} = \eta(\alpha),\alpha\in (0,1)\}$, then $\mathcal{C}_1$ and $\mathcal{C}_2$ must have at least one intersection, noted as $(\widehat{\alpha}_A,\widehat{\zeta}^{00})$. %, and $\widehat{\alpha}_A\leq \widehat{\alpha}_B$ must hold under Condition \ref{con:transition}(i), while $\widehat{\alpha}_A\geq \widehat{\alpha}_B$ must hold under Condition \ref{con:transition}(ii). 
However, in order for $(\widehat{\alpha}_A,\widehat{\zeta}^{00})$ to be a valid equilibrium of the system for scenario $A$, it must satisfy $\widehat{\alpha}_A+\widehat{\zeta}^{00}\leq 1$. We show it in the following.  

Sum up above balanced equations regarding $\alpha$ and $\zeta^{00}$ gives
\begin{eqnarray*}
\widehat{\alpha}_A+\widehat{\zeta}^{00}&=& [T_{11}-T_{01}+(1-T_{11})\mathbb{G}_1(\theta) + (T_{01}-1)\mathbb{G}_{01}(\theta)]\widehat{\alpha}_A \\&&+ (\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{01}-1)\widehat{\zeta}^{00} + T_{01} + (1-T_{01})\mathbb{G}_{01}(\theta)\\
&=&T_{01} + (1-T_{01})\mathbb{G}_{01}(\theta)(1-\widehat{\alpha}_A-\widehat{\zeta}^{00}) + (1-T_{01})\mathbb{G}_{00}(\theta)\widehat{\zeta}^{00} \\&&+ \widehat{\alpha}_A (T_{11}-T_{01}+(1-T_{11})\mathbb{G}_{1}(\theta))\\
&\leq & T_{01} +\max \{(1-T_{01})\mathbb{G}_{01}(\theta),(1-T_{01})\mathbb{G}_{00}(\theta),T_{11}-T_{01}+(1-T_{11})\mathbb{G}_{1}(\theta) \}
\end{eqnarray*}
Since 
\begin{eqnarray*}
T_{01} + (1-T_{01})\mathbb{G}_{01}(\theta) &\leq& T_{01} + (1-T_{01}) = 1\\
T_{01} + (1-T_{01})\mathbb{G}_{00}(\theta) &\leq & T_{01} + (1-T_{01}) = 1\\
T_{01} + T_{11}-T_{01}+(1-T_{11})\mathbb{G}_{1}(\theta) = T_{11}+(1-T_{11})\mathbb{G}_{1}(\theta) &\leq & T_{11}+(1-T_{11}) = 1
\end{eqnarray*}
It implies that $\widehat{\alpha}_A+\widehat{\zeta}^{00}\leq 1$.

Scenario $B$ has the equilibrium if there is $\alpha$ such that the following holds:
\begin{eqnarray*}
\frac{1}{\alpha}- 1 = \frac{1-T_{11}(1-\mathbb{G}_{1}(\theta_B(\alpha)))-T_{10}\mathbb{G}_{1}(\theta_B(\alpha))}{T_{01}(1-\mathbb{G}_{01}(\theta_B(\alpha)))+T_{00}\mathbb{G}_{01}(\theta_B(\alpha))} = h_B(\theta_B(\alpha))
\end{eqnarray*}
Under conditions of Theorem \ref{thm:unique_equilibrium}, scenario $B$ has unique equilibrium $\widehat{\alpha}_B$. 

Consider case when $\mathbb{G}_{01}(\theta) \leq \mathbb{G}_{00}(\theta)$ and ${G}_{01}(\widehat{x}) = {G}_{00}(\widehat{x})$, ${G}_{01}(x) < {G}_{00}(x), \forall x < \widehat{x}$, ${G}_{01}(x) > {G}_{00}(x), \forall x > \widehat{x}$.

Define $f_B(\theta,\alpha) \coloneqq \frac{G_{01}(\theta)}{G_1(\theta)}\frac{1-\alpha}{\alpha}$ and $f_A(\theta,\alpha,\zeta^{00}) \coloneqq \frac{G_{00}(\theta)}{G_1(\theta)}\frac{\zeta^{00}}{\alpha} + \frac{G_{01}(\theta)}{G_1(\theta)}\frac{1-\alpha-\zeta^{00}}{\alpha}$. Then given $\alpha,\zeta^{00}$, qualification profiles under scenarios $A$ and $B$ are $\gamma_A(\theta) = \frac{1}{1+ f_A(\theta,\alpha,\zeta^{00})}$ and $\gamma_B(\theta) = \frac{1}{1+ f_B(\theta,\alpha)}$, respectively. 

Because ${G}_{01}(\widehat{x}) = {G}_{00}(\widehat{x})$, ${G}_{01}(x) < {G}_{00}(x), \forall x < \widehat{x}$, ${G}_{01}(x) > {G}_{00}(x), \forall x > \widehat{x}$, given any $\alpha,\zeta^{00}$, we have $f_A(\theta,\alpha,\zeta^{00}) > f_B(\theta,\alpha), \forall \theta < \widehat{x}$, $f_A(\theta,\alpha,\zeta^{00}) < f_B(\theta,\alpha), \forall \theta > \widehat{x}$ and $f_A(\widehat{x},\alpha,\zeta^{00}) = f_B(\widehat{x},\alpha)$. By optimal equation \eqref{eq:opt_fair_policy}, given any $\alpha,\zeta^{00}$, the unconstrained optimal policies $\theta_A(\alpha,\zeta^{00})$, $\theta_B(\alpha)$ under two scenarios satisfy $$\gamma_A(\theta_A(\alpha,\zeta^{00})) = \gamma_B(\theta_B(\alpha)) = \frac{u_-}{u_++u_-}\Longleftrightarrow  f_A(\theta_A(\alpha,\zeta^{00}),\alpha,\zeta^{00})  = f_B(\theta_B(\alpha),\alpha)=\frac{u_+}{u_-}. $$
Denote $\beta(\widehat{x},\alpha) \coloneqq \frac{G_{01}(\widehat{x})}{G_1(\widehat{x})}\frac{1-\alpha}{\alpha} = \frac{G_{00}(\widehat{x})}{G_1(\widehat{x})}\frac{1-\alpha}{\alpha}$.
It implies that $ \theta_A(\alpha,\zeta^{00}) > \theta_B(\alpha)$ iff $\frac{u_+}{u_-}> \beta(\widehat{x},\alpha)$; $ \theta_A(\alpha,\zeta^{00}) < \theta_B(\alpha)$ iff $\frac{u_+}{u_-} <\beta(\widehat{x},\alpha)$.

Since $\beta(\widehat{x},\alpha)$ is strictly decreasing from $+\infty$ to 0 over $\alpha \in [0,1]$, define  $\overline{\alpha} \coloneqq \frac{1}{1+\frac{u_+}{u_-}\frac{G_{1}(\widehat{x})}{G_{01}(\widehat{x})} }$ such that $\frac{u_+}{u_-} =\beta(\widehat{x},\overline{\alpha})$. Then $\frac{u_+}{u_-} <\beta(\widehat{x},\alpha), \forall \alpha \in [0,\overline{\alpha})$ and $\frac{u_+}{u_-} >\beta(\widehat{x},\alpha), \forall \alpha \in (\overline{\alpha},1]$.

Because under Condition \ref{con:transition}\ref{con:transition_II}, we have $\frac{1}{\widehat{\alpha}_B } - 1 \in (\frac{1-T_{11}}{T_{01}},\frac{1-T_{10}}{T_{00}} )$. If $\frac{u_+}{u_-}>\frac{G_{01}(\widehat{x})}{G_{1}(\widehat{x})}\frac{1-T_{10}}{T_{00}}$, then $\frac{u_+}{u_-} >\frac{G_{01}(\widehat{x})}{G_{1}(\widehat{x})}(\frac{1}{\widehat{\alpha}_B } - 1)=\beta(\widehat{x},\widehat{\alpha}_B)$ holds so that $\theta_A(\widehat{\alpha}_B,\zeta^{00}) > \theta_B(\widehat{\alpha}_B ),\forall \zeta^{00}$ and $\widehat{\alpha}_B\in(\overline{\alpha},1]$. It further implies that $\theta_A({\alpha},\zeta^{00}) > \theta_B({\alpha} ),\forall \zeta^{00}, \alpha\in [\widehat{\alpha}_B,1]$.
Moreover, $(\mathbb{G}_{01}(\theta)-\mathbb{G}_{00}(\theta))(T_{01}-T_{00})\zeta^{00} < 0$ holds $\forall \zeta^{00},\theta$. Therefore, we have $$h_A(\theta_A(\alpha,\zeta^{00}) ) > h_B(\theta_B(\alpha) ) \geq h_B(\theta_B(\widehat{\alpha}_B) )= \frac{1}{\widehat{\alpha}_B }-1, \forall \alpha\in [\widehat{\alpha}_B,1], \forall \zeta^{00}.$$
It implies that $h_A(\theta_A(\alpha,\zeta^{00}) )$ has no intersection with $\frac{1}{\alpha}-1$ over $\alpha\in [\widehat{\alpha}_B,1]$. Therefore, $\widehat{\alpha}_A < \widehat{\alpha}_B$.

 

Similarly, under Condition \ref{con:transition}\ref{con:transition_I}, we have $\frac{1}{\widehat{\alpha}_B } - 1 \in (\frac{1-T_{10}}{T_{00}},\frac{1-T_{11}}{T_{01}} )$. if $\frac{u_+}{u_-}>\frac{G_{01}(\widehat{x})}{G_{1}(\widehat{x})}\frac{1-T_{11}}{T_{01}}$, then $\theta_A(\widehat{\alpha}_B,\zeta^{00}) > \theta_B(\widehat{\alpha}_B ),\forall \zeta^{00}$ and $\widehat{\alpha}_B\in(\overline{\alpha},1]$ hold. It further implies $\theta_A({\alpha},\zeta^{00}) > \theta_B({\alpha} ),\forall \zeta^{00}, \alpha\in [\widehat{\alpha}_B,1]$. Therefore, we have $$h_A(\theta_A(\alpha,\zeta^{00}) ) < h_B(\theta_B(\alpha) ) \leq h_B(\theta_B(\widehat{\alpha}_B) )= \frac{1}{\widehat{\alpha}_B }-1, \forall \alpha\in [\widehat{\alpha}_B,1], \forall \zeta^{00}.$$
Therefore, $\widehat{\alpha}_A > \widehat{\alpha}_B$.


Using the similar analysis, the case when $\mathbb{G}_{01}(\theta) \geq \mathbb{G}_{00}(\theta)$ and ${G}_{01}(\widehat{x}) = {G}_{00}(\widehat{x})$, ${G}_{01}(x) > {G}_{00}(x), \forall x < \widehat{x}$, ${G}_{01}(x) < {G}_{00}(x), \forall x > \widehat{x}$ can also be proved and is omitted.



 

\end{proof}

\paragraph{The Proof of Theorem \ref{thm:generation1}.}
\begin{proof}
In the proof, let $G_{01}(x) = G_{00}(x) = G_0(x)$ and remove subscript $A$ to simplify the notation, i.e., ${G}_{1a}^A(\theta)\coloneqq {G}_{1a}(\theta)$, $\forall a\in\{0,1\}$. 

Under Assumption \ref{ass:3} and the case when $G_{01}(x) = G_{00}(x) = G_{0}(x)$, $G_{11}(x) \neq G_{10}(x)$, use the fact that $\zeta^{01}_t + \zeta^{00}_t = 1-\alpha_t$, $\zeta^{11}_t + \zeta^{10}_t +\zeta^{01}_t + \zeta^{00}_t = 1$, dynamics of qualification rate can be simplified as follows, where $\theta_t$ is the threshold of the policy at $t$. 
\begin{eqnarray*}
1-\alpha_{t+1} &=& \Big[(1-T_{10})(1-\mathbb{G}_{0}(\theta_t))+(1-T_{00})\mathbb{G}_{0}(\theta_t)- (1-T_{11})(1-\mathbb{G}_{10}(\theta_t))\\&&-(1-T_{10})\mathbb{G}_{10}(\theta_t)\Big](1-\alpha_t) + (T_{11}-T_{10})(\mathbb{G}_{11}(\theta_t)-\mathbb{G}_{10}(\theta_t))\zeta^{11}_t\\&& + (1-T_{11})(1-\mathbb{G}_{10}(\theta_t)) + (1-T_{10})\mathbb{G}_{10}(\theta_t)\\
\zeta^{11}_{t+1} &=& \Big[T_{01}(1-\mathbb{G}_0(\theta_t))-T_{11}(1-\mathbb{G}_{10}(\theta_t))\Big](1-\alpha_t)\\&& + T_{11}(1-\mathbb{G}_{10}(\theta_t)) + T_{11}(\mathbb{G}_{10}(\theta_t)-\mathbb{G}_{11}(\theta_t))\zeta^{11}_t
\end{eqnarray*}
and qualification profile is reduced to $\gamma_t(x) =  \frac{1}{1 + 
\frac
{(1-\alpha_t)G_{0}(x)}
{G_{10}(x) \zeta^{10}_t+G_{11}(x) \zeta^{11}_t}
}$.

Scenario $A$ has the equilibrium if there exists $\alpha$, $\zeta^{11}$ such that the following holds:
\begin{eqnarray*}
1-\alpha &=& \Big[(1-T_{10})(1-\mathbb{G}_{0}(\theta))+(1-T_{00})\mathbb{G}_{0}(\theta)- (1-T_{11})(1-\mathbb{G}_{10}(\theta))\\&&-(1-T_{10})\mathbb{G}_{10}(\theta)\Big](1-\alpha) + (T_{11}-T_{10})(\mathbb{G}_{11}(\theta)-\mathbb{G}_{10}(\theta))\zeta^{11}\\&& + (1-T_{11})(1-\mathbb{G}_{10}(\theta)) + (1-T_{10})\mathbb{G}_{10}(\theta)\\
\zeta^{11} &=& \Big[T_{01}(1-\mathbb{G}_0(\theta))-T_{11}(1-\mathbb{G}_{10}(\theta))\Big](1-\alpha)\\&& + T_{11}(1-\mathbb{G}_{10}(\theta)) + T_{11}(\mathbb{G}_{10}(\theta)-\mathbb{G}_{11}(\theta))\zeta^{11}
\end{eqnarray*}
Re-organize above equations,
\begin{eqnarray*}
\frac{1}{1-\alpha} - 1 &= & h_A(\theta_A(\zeta^{11},\alpha)) \\&=& \frac{1-(1-T_{01})(1-\mathbb{G}_0(\theta))-(1-T_{00})\mathbb{G}_0(\theta)-(T_{11}-T_{10})(\mathbb{G}_{11}(\theta)-\mathbb{G}_{10}(\theta))\zeta^{11}}{(1-T_{11})(1-\mathbb{G}_{10}(\theta))+ (1-T_{10})\mathbb{G}_{10}(\theta)+(T_{11}-T_{10})(\mathbb{G}_{11}(\theta)-\mathbb{G}_{10}(\theta))\zeta^{11}} \\
\zeta^{11} &=&  \frac{[T_{01}(1-\mathbb{G}_0(\theta))-T_{11}(1-\mathbb{G}_{10}(\theta))](1-\alpha) + T_{11}(1-\mathbb{G}^{01}(\theta))}{1-T_{11}(\mathbb{G}_{01}(\theta)-\mathbb{G}_{11}(\theta))} = g_A(\theta_A(\zeta^{11},\alpha))
\end{eqnarray*}
where $\theta \coloneqq \theta_A(\zeta^{11},\alpha)$ for simplification.
Given any $\zeta^{11}$, $h_A(\theta(\zeta^{11},\alpha))$ is continuous in $\alpha$, there exists at least one $\overline{\alpha} \coloneqq \psi(\zeta^{11})$ such that $\frac{1}{1-\overline{\alpha}}-1 = h_A(\theta_A(\zeta^{11},\overline{\alpha}))$ holds. 


Given any $\alpha\in [0,1]$, $g_A(\theta_A(\zeta^{11},\alpha))\in (0,1)$ is continuous in $\zeta^{11}$, while $\zeta^{11}$ is strictly increasing from 0 to 1. Therefore, there exists at least one $\overline{\zeta}^{11}\coloneqq \eta(\alpha)$ such that $\overline{\zeta}^{11} =  g_A(\theta_A(\zeta^{11},\alpha))$. 

Consider a 2D plane $\{(\alpha,\zeta^{11}):\zeta^{11}\in [0,1],\alpha\in[0,1]\}$, two sets of curves $\mathcal{C}_1 = \{(\alpha,\zeta^{11}):\alpha = \psi(\zeta^{11}),\zeta^{11}\in (0,1)\}$ and $\mathcal{C}_2 = \{(\alpha,\zeta^{11}):\zeta^{11} = \eta(\alpha),\alpha\in (0,1)\}$, then $\mathcal{C}_1$ and $\mathcal{C}_2$ must have at least one intersection, noted as $(\widehat{\alpha}_A,\widehat{\zeta}^{11})$. However, in order for $(\widehat{\alpha}_A,\widehat{\zeta}^{11})$ to be a valid equilibrium of the system for scenario $A$, it must satisfy $0\leq 1-\widehat{\alpha}_A+\widehat{\zeta}^{11}\leq 1$. We show it in the following.  

Sum up above balanced equations regarding $1-\alpha$ and $\zeta^{11}$ gives
\begin{eqnarray*}
&&1-\widehat{\alpha}_A+\widehat{\zeta}^{11}\\& =& (T_{10}\mathbb{G}_{10}(\theta)-T_{00}\mathbb{G}_{0}(\theta))(1-\widehat{\alpha}_A) - T_{10}(\mathbb{G}_{11}(\theta)-\mathbb{G}_{10}(\theta))\widehat{\zeta}^{11} + 1-T_{10}\mathbb{G}_{10}(\theta)\\
&= & 1 - \Big(\mathbb{G}_{10}(\theta)T_{10}(\widehat{\alpha}_A - \widehat{\zeta}^{11}) +  T_{00}\mathbb{G}_{0}(\theta)(1-\widehat{\alpha}_A) + T_{10}\mathbb{G}_{11}(\theta)\widehat{\zeta}^{11}\Big)
\end{eqnarray*}

Since $\mathbb{G}_{10}(\theta)T_{10}(\widehat{\alpha}_A - \widehat{\zeta}^{11}) +  T_{00}\mathbb{G}_{0}(\theta)(1-\widehat{\alpha}_A) + T_{10}\mathbb{G}_{11}(\theta)\widehat{\zeta}^{11} $ is the convex combination of $\mathbb{G}_{10}(\theta)T_{10}\in [0,1]$, $T_{00}\mathbb{G}_{0}(\theta)\in [0,1]$ and $T_{10}\mathbb{G}_{11}(\theta)\in [0,1]$. Therefore, $1-\widehat{\alpha}_A+\widehat{\zeta}^{11} \in [0,1]$.

Scenario $B$ has the equilibrium if there is $\alpha$ such that the following holds:
$$  \frac{1}{1-\alpha} - 1=\frac{1-(1-T_{01})(1-\mathbb{G}_0(\theta_B(\alpha)))-(1-T_{00})\mathbb{G}_0(\theta_B(\alpha))}{(1-T_{11})(1-\mathbb{G}_{10}(\theta_B(\alpha)))+ (1-T_{10})\mathbb{G}_{10}(\theta_B(\alpha))} = h_B(\theta_B(\alpha)). $$
Under conditions of Theorem \ref{thm:unique_equilibrium}, scenario $B$ has unique equilibrium $\widehat{\alpha}_B$. 


Consider the case when $\mathbb{G}_{11}(x) \leq \mathbb{G}_{10}(x),\forall x$ and ${G}_{11}(\widehat{x}) = {G}_{10}(\widehat{x})$, ${G}_{11}(x) < {G}_{10}(x), \forall x < \widehat{x}$, ${G}_{11}(x) > {G}_{10}(x), \forall x > \widehat{x}$. 


Define $f_B(\theta,\alpha) \coloneqq \frac{G_{0}(\theta)}{G_{10}(\theta)}\frac{1-\alpha}{\alpha}$ and $f_A(\theta,\alpha,\zeta^{11}) \coloneqq \frac{G_{0}(\theta)(1-\alpha)}{G_{10}(\theta)(1-\zeta^{11}-\alpha) + G_{11}(\theta)\zeta^{11}}$. Then given $\alpha,\zeta^{11}$, qualification profiles under scenarios $A$ and $B$ are $\gamma_A(\theta) = \frac{1}{1+ f_A(\theta,\alpha,\zeta^{11})}$ and $\gamma_B(\theta) = \frac{1}{1+ f_B(\theta,\alpha)}$, respectively. Given any $\alpha,\zeta^{11}$, we have $f_A(\theta,\alpha,\zeta^{11}) > f_B(\theta,\alpha), \forall \theta < \widehat{x}$, $f_A(\theta,\alpha,\zeta^{11}) < f_B(\theta,\alpha), \forall \theta > \widehat{x}$ and $f_A(\widehat{x},\alpha,\zeta^{11}) = f_B(\widehat{x},\alpha)$. By optimal equation \eqref{eq:opt_fair_policy}, given any $\alpha,\zeta^{11}$, the unconstrained optimal policies $\theta_A(\alpha,\zeta^{11})$, $\theta_B(\alpha)$ under two scenarios satisfy $$\gamma_A(\theta_A(\alpha,\zeta^{11})) = \gamma_B(\theta_B(\alpha)) = \frac{u_-}{u_++u_-}\Longleftrightarrow  f_A(\theta_A(\alpha,\zeta^{11}),\alpha,\zeta^{11})  = f_B(\theta_B(\alpha),\alpha)=\frac{u_+}{u_-}. $$
Denote $\beta(\widehat{x},\alpha) \coloneqq \frac{G_{0}(\widehat{x})}{G_{10}(\widehat{x})}\frac{1-\alpha}{\alpha} = \frac{G_{0}(\widehat{x})}{G_{11}(\widehat{x})}\frac{1-\alpha}{\alpha}$.
It implies that $ \theta_A(\alpha,\zeta^{11}) > \theta_B(\alpha)$ iff $\frac{u_+}{u_-}> \beta(\widehat{x},\alpha)$; $ \theta_A(\alpha,\zeta^{11}) < \theta_B(\alpha)$ iff $\frac{u_+}{u_-}<\beta(\widehat{x},\alpha)$.

Since $\beta(\widehat{x},\alpha)$ is strictly decreasing from $+\infty$ to 0 over $\alpha \in [0,1]$, define  $\overline{\alpha} \coloneqq \frac{1}{1+\frac{u_+}{u_-}\frac{G_{10}(\widehat{x})}{G_{0}(\widehat{x})} }$ such that $\frac{u_+}{u_-} =\beta(\widehat{x},\overline{\alpha})$. Then $\frac{u_+}{u_-} <\beta(\widehat{x},\alpha), \forall \alpha \in [0,\overline{\alpha})$ and $\frac{u_+}{u_-} >\beta(\widehat{x},\alpha), \forall \alpha \in (\overline{\alpha},1]$.

Because under Condition \ref{con:transition}\ref{con:transition_II}, we have $\frac{1}{\widehat{\alpha}_B } - 1 \in (\frac{1-T_{11}}{T_{01}},\frac{1-T_{10}}{T_{00}} )$. If $\frac{u_+}{u_-}<\frac{G_{0}(\widehat{x})}{G_{10}(\widehat{x})}\frac{1-T_{11}}{T_{01}}$, then $\frac{u_+}{u_-} <\frac{G_{0}(\widehat{x})}{G_{10}(\widehat{x})}(\frac{1}{\widehat{\alpha}_B } - 1)=\beta(\widehat{x},\widehat{\alpha}_B)$ holds so that $\theta_A(\widehat{\alpha}_B,\zeta^{11}) < \theta_B(\widehat{\alpha}_B ),\forall \zeta^{11}$ and $\widehat{\alpha}_B\in[0,\overline{\alpha})$. It further implies that $\theta_A({\alpha},\zeta^{11}) < \theta_B({\alpha} ),\forall \zeta^{11}, \alpha\in [0,\widehat{\alpha}_B]$.
Moreover, $(T_{11}-T_{10})(\mathbb{G}_{11}(\theta)-\mathbb{G}_{10}(\theta))\zeta^{11}<0$ holds $\forall \zeta^{11},\theta$. Therefore, we have $$h_A(\theta_A(\alpha,\zeta^{11}) ) > h_B(\theta_B(\alpha) ) \geq h_B(\theta_B(\widehat{\alpha}_B) )= \frac{1}{\widehat{\alpha}_B }-1, \forall \alpha\in [0,\widehat{\alpha}_B], \forall \zeta^{11}.$$
It implies that $h_A(\theta_A(\alpha,\zeta^{11}) )$ has no intersection with $\frac{1}{1-\alpha}-1$ over $\alpha\in [0,\widehat{\alpha}_B]$. Therefore, $\widehat{\alpha}_A > \widehat{\alpha}_B$.

Similarly, under Condition \ref{con:transition}\ref{con:transition_I}, we have $\frac{1}{\widehat{\alpha}_B } - 1 \in (\frac{1-T_{10}}{T_{00}},\frac{1-T_{11}}{T_{01}} )$. if $\frac{u_+}{u_-}<\frac{G_{0}(\widehat{x})}{G_{10}(\widehat{x})}\frac{1-T_{10}}{T_{00}}$, then $\theta_A(\widehat{\alpha}_B,\zeta^{11}) < \theta_B(\widehat{\alpha}_B ),\forall \zeta^{11}$ and $\widehat{\alpha}_B\in[0,\overline{\alpha})$ hold. It further implies $\theta_A({\alpha},\zeta^{11}) < \theta_B({\alpha} ),\forall \zeta^{11}, \alpha\in [0,\widehat{\alpha}_B]$. Therefore, we have $$h_A(\theta_A(\alpha,\zeta^{00}) ) < h_B(\theta_B(\alpha) ) \leq h_B(\theta_B(\widehat{\alpha}_B) )= \frac{1}{\widehat{\alpha}_B }-1, \forall \alpha\in [0,\widehat{\alpha}_B], \forall \zeta^{11}.$$
Therefore, $\widehat{\alpha}_A < \widehat{\alpha}_B$.

Using the similar analysis, the case when $\mathbb{G}_{11}(x) \geq \mathbb{G}_{10}(x), \forall x$ and ${G}_{11}(\widehat{x}) = {G}_{10}(\widehat{x})$, ${G}_{11}(x) > {G}_{10}(x), \forall x < \widehat{x}$, ${G}_{11}(x) < {G}_{10}(x), \forall x > \widehat{x}$ can also be proved and is omitted.

\end{proof}
